What is it like to program with artificial intelligence?

Large language models, such as OpenAI's codex and Deepmind's AlphaCode, can generate code to solve a variety of problems expressed in natural language. This technology has already been commercialised in at least one widely-used programming editor extension: GitHub Copilot. In this paper, we explore how programming with large language models (LLM-assisted programming) is similar to, and differs from, prior conceptualisations of programmer assistance. We draw upon publicly available experience reports of LLM-assisted programming, as well as prior usability and design studies. We find that while LLM-assisted programming shares some properties of compilation, pair programming, and programming via search and reuse, there are fundamental differences both in the technical possibilities as well as the practical experience. Thus, LLM-assisted programming ought to be viewed as a new way of programming with its own distinct properties and challenges. Finally, we draw upon observations from a user study in which non-expert end user programmers use LLM-assisted tools for solving data tasks in spreadsheets. We discuss the issues that might arise, and open research challenges, in applying large language models to end-user programming, particularly with users who have little or no programming expertise.

==> sec_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
[Maybe we don't need a discussion]
% Advait's old crazy ramblings
% Programming with AI assistance as a Chinese room

% Reuse of code and spreadsheets as Chinese room

% Why is programming an activity with primacy unlike other human-machine systems?

% How does it relate to ai as material.

% Other conceptualisations of ai, eg as cognitive extension 

% Why is programming with high level apis not already like a Chinese room.

% scope of assistance (short snippets to full program) and role of programmer (helmsman, collage artist, debugger, finisher/fine-tuner)

% dependency on outcome (whether the program needs to be robustly reused, or whether it is just a one-use thing and can have errors that can be ignored or compensated for in other ways).

% AI as facilitating institutionalised plagiarism (see Blackwell)

% What is the distinction between an end user and a programmer that reuses code?

% A new practice of programming? (see Blackwell's practices of programming)


% Good, Judith, and Kate Howland. "Programming language, natural language? Supporting the diverse computational activities of novice programmers." Journal of Visual Languages & Computing 39 (2017): 78-92.

% Dijkstra, Edsger W. "On the foolishness of" natural language programming"." In Program construction, pp. 51-53. Springer, Berlin, Heidelberg, 1979.

% See also, Mary’s room thought experiment. Neuroscientist who can’t see colour. Knowledge argument.

% Instrument vs machine, from Marx's 'fragment on machines' (https://thenewobjectivity.com/pdf/marx.pdf):

% "Not as with the instrument, which the worker animates and makes into his organ with his skill and strength, and whose handling therefore depends on his virtuosity. Rather, it is the machine which possesses skill and strength in place of the worker, is itself the virtuoso, with a soul of its own in the mechanical laws acting through it; and it consumes coal, oil etc. (mati\`eres instrumentales), just as the worker consumes food, to keep up its perpetual motion. The worker's activity, reduced to a mere abstraction of activity, is determined and regulated on all sides by the movement of the machinery, and not the opposite."
